Improved Customer Transaction Classification using Semi-Supervised Knowledge Distillation

In pickup and delivery services, transaction classification based on customer provided free text is a challenging problem. It involves the association of a wide variety of customer inputs to a fixed set of categories while adapting to the various customer writing styles. This categorization is important for the business: it helps understand the market needs and trends, and also assist in building a personalized experience for different segments of the customers. Hence, it is vital to capture these category information trends at scale, with high precision and recall. In this paper, we focus on a specific use-case where a single category drives each transaction. We propose a cost-effective transaction classification approach based on semi-supervision and knowledge distillation frameworks. The approach identifies the category of a transaction using free text input given by the customer. We use weak labelling and notice that the performance gains are similar to that of using human-annotated samples. On a large internal dataset and on 20Newsgroup dataset, we see that RoBERTa performs the best for the categorization tasks. Further, using an ALBERT model (it has 33x fewer parameters vis-a-vis parameters of RoBERTa), with RoBERTa as the Teacher, we see a performance similar to that of RoBERTa and better performance over unadapted ALBERT. This framework, with ALBERT as a student and RoBERTa as teacher, is further referred to as R-ALBERT in this paper. The model is in production and is used by business to understand changing trends and take appropriate decisions.

==> dataset.tex <==
\section{Dataset}

We make use of a large internal dataset spread across different time windows and different annotation strategies as shown in table \ref{tab:my-table-data}. We only consider the transactions which has a customer text input associated with it.

Following are the list of 10 categories considered for the experiments -  \{'Food', 'Grocery', 'Package', 'Medicines', 'Household Items', 'Cigarettes', 'Clothes', 'Electronics', 'Keys', 'Documents/Books'\}

\textbf{\textit{Manual labelling}} strategy refers to the labels assigned to each transaction by a team of subject matter experts and \textbf{\textit{Weak labelling}} refers to the labels generated by the RoBERTa model, trained on ``Train 1''. All the tests are done on a \textbf{\textit{separate}} held out test set.

\begin{table}[]{
\begin{tabular}{|l|l|l|p{2cm}|}
\hline
\textbf{Name} & \textbf{Duration} & \textbf{Size} & \textbf{Annotation Strategy} \\ \hline
     Train 1 &  Sept - Dec       & 41,539     & Manual                    \\ \hline
    %  Train 2 & April      &18,160   &  Manual                        \\ \hline
     Train 2 & Jan - Apr        &   93,820    & Weak labels                   \\ \hline
     Test 1 & April      &1,999   &  Manual                        \\ \hline

\end{tabular}
}
\caption{Dataset Description}
\label{tab:my-table-data}
\end{table}
